IOI: Decoupling Kinematics and Physics for Interactive World Models

Developing generalist embodied agents requires interactive environments providing visually realistic feedback and accurate action-conditioned dynamics. Interactive world models address this by simulating such complex dynamics. However, purely data-driven methods struggle to ensure precise control alignment and physically plausible visual feedback due to a lack of explicit structural constraints. To address this, we propose IOI, a hybrid interactive world model integrating analytical kinematic priors with learned physical dynamics. Unlike data-driven approaches prone to spatiotemporal drift, IOI introduces explicit kinematic guidance, computing forward kinematics from action sequences for accurate motion trajectories. These trajectories are rendered into synchronized front, side, and top orthographic projections, eliminating the need for extrinsic camera calibration. A Multi-view Kinematic Aggregation and Injection module fuses these geometric cues and injects them into the video generator, providing geometry-consistent guidance. Conditioning video generation on these deterministic trajectories establishes a synergy between the analytical simulator and the world model. Decoupling deterministic motion into the kinematic prior frees the generator to model stochastic physical interactions. Experiments on the RoboTwin benchmark validate IOI across kinematic fidelity, out-of-distribution (OOD) generalization, and policy evaluation. IOI achieves state-of-the-art simulation performance and robust zero-shot generalization to unseen OOD tasks. Furthermore, IOI serves as a reliable policy evaluator, yielding success rates closely aligning with ground-truth physics simulators. On real-world platforms, policies trained on IOI-synthesized data match those trained on teleoperation demonstrations, solidifying its practical value for embodied policy learning.

==> sec/0_abstract.tex <==
\begin{abstract}
Developing generalist embodied agents demands scalable and interactive environments that provide both visually realistic feedback and accurate action-conditioned dynamics for policy learning and evaluation. Interactive world models offer a promising paradigm to address this challenge by simulating complex action-conditioned dynamics. However, existing methods often struggle to simultaneously ensure precise control alignment and physically plausible visual feedback, primarily stemming from the absence of explicit structural constraints in purely data-driven frameworks. To address this limitation, we propose IOI, a hybrid interactive world model that integrates analytical kinematic priors with learned physical dynamics. Unlike purely data-driven generation approaches prone to spatiotemporal drift, IOI introduces explicit kinematic guidance, computing forward kinematics from action sequences to obtain accurate motion trajectories. These trajectories are rendered into synchronized front, side, and top orthographic projections, which eliminate the need for extrinsic camera calibration to align rendered motions with observed scenes. A lightweight yet effective Multi-view Kinematic Aggregation and Injection module then fuses these multi-view geometric cues and injects them into the video generator, providing geometry-consistent and view-invariant guidance. By conditioning video generation on deterministic kinematic trajectories, IOI establishes a principled synergy between the analytical simulator and the world model. By decoupling deterministic embodiment motion into the kinematic prior, the generator's representational capacity is fully dedicated to modeling stochastic physical interactions and environmental dynamics. 
Extensive experiments on the RoboTwin benchmark comprehensively validate IOI across three critical dimensions: kinematic fidelity, out-of-distribution (OOD) generalization, and policy evaluation. IOI achieves state-of-the-art simulation performance, while demonstrating robust zero-shot generalization to unseen OOD tasks. Furthermore, IOI serves as a highly reliable policy evaluator, yield success rates that closely align with ground-truth physics simulators. On real-world platforms, policies trained on IOI-synthesized data match those trained on teleoperation demonstrations, solidifying its practical value for embodied policy learning.
% Extensive experiments on the RoboTwin benchmark demonstrate that IOI achieves state-of-the-art performance, outperforming prior methods by a large margin of 36.47\% in FVD. On real-world platforms, policies trained on IOI-synthesized data match those trained on teleoperation demonstrations, further validating IOI as a reliable evaluator for embodied policy learning.
\end{abstract}
